Teach Me to Explain: A Review of Datasets for Explainable Natural Language Processing

Explainable NLP (ExNLP) has increasingly focused on collecting human-annotated textual explanations. These explanations are used downstream in three ways: as data augmentation to improve performance on a predictive task, as supervision to train models to produce explanations for their predictions, and as a ground-truth to evaluate model-generated explanations. In this review, we identify 65 datasets with three predominant classes of textual explanations (highlights, free-text, and structured), organize the literature on annotating each type, identify strengths and shortcomings of existing collection methodologies, and give recommendations for collecting ExNLP datasets in the future.

==> main_takeaways.tex <==
\section{Main Takeaways}
\label{appendix:takeaways}
\paragraph{Available human-annotated highlights are not necessarily sufficient nor comprehensive (\sect{sec:collecting_highlights}).}
\begin{compactenum}
\item[{1.}] It is important to precisely report how explanations were collected, e.g., by providing a screenshot of the annotation interface,  giving access to it, or giving the annotation instructions word for word.
\item[{2.}] Sufficiency is necessary for highlights, and \exnlp researchers should avoid human-annotated highlights with low sufficiency for evaluating and developing highlights.
\item[{3.}] Comprehensiveness is not necessary for a valid highlight, but it is a means to quantify faithfulness.
\item[{4.}] Non-comprehensive human-annotated highlights cannot be used to automatically evaluate plausibility of highlights that are constrained to be comprehensive. In this case, \exnlp researchers should collect and use comprehensive human-annotated highlights.
\item[{5.}] When deciding which datasets to use, \exnlp researchers should not make post-hoc estimates of comprehensiveness of human-annotated highlights from datasets' general descriptions since that is error-prone.
\item[{6.}] \exnlp researchers should be careful to not popularize their data collection decisions as universally necessary. We advocate for documenting all constraints on collected explanations in a datasheet, highlighting whether each constraint is necessary for explanation to be valid or not, and noting how each constraint might affect modeling and evaluation to the best of the author's knowledge.
\end{compactenum}

\paragraph{Entirely free-text explanations are not always the most natural (\sect{sec:case_study_cose_esnli}).}
\begin{compactenum}
\item[{7.}] \exnlp researchers should study how people define and generate explanations for the task before collecting free-text explanations. If pilot studies show that explanations are naturally structured, embrace the structure. 
\item[{8.}] There is no all-encompassing definition of explanation. Thus, \exnlp researchers could consult domain experts or follow literature from other fields to define an appropriate explanation form, and these matters should be open for debate on a given task. 
\end{compactenum}

\paragraph{Getting the most out of data collection (\sect{sec:quality}, \sect{sec:related_quality}).}
\begin{compactenum}
\item[{9.}] Using a \CollectAndEdit method can reduce individual annotator biases, perform quality control, and potentially reduce dataset artifacts.
\item[{10.}] For quality control, we discuss teaching and testing the underlying task (\sect{sec:teaching_task}) and addressing ambiguity (\sect{subsec:unsure}).
\item[{11.}] To increase annotation diversity, we discuss the importance of a large set of annotators (\sect{sec:num_annotators}), multiple annotations per instance (\sect{sec:num_annotations}), and collecting explanations that are most useful to the needs of end-users (\sect{sec:coverage}).
\item[{13.}] Reporting inter-annotator agreement with plausibility of annotated explanations is useful to known whether there is a natural diversity of explanations for the task and should the diversity be considered for modeling and evaluation.
\item[{14.}] \exnlp challenges discussed in \sect{sec:related_quality}, such as the automatic measurement of meaning overlap between two explanations, are similar to fundamental NLP challenges outside of \exnlp. NLP research (especially prior to the emergence of end-to-end black-box neural NLP) might bear on these questions.
\end{compactenum}

==> neurips_2021_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} We make a best-effort to justify our scope clearly in \sect{sec:introduction}. We also include additional discussion of the definition of explanation in XAI and datasets not included under this definition in \autoref{sec:definition}.
  \item Did you discuss any potential negative societal impacts of your work? \answerYes{} In \sect{sec:quality} and \sect{sec:related_quality}, we discuss reasons for dataset artifacts that are related to amplifying social bias. Namely, we acknowledge that social expectations and socio-cultural background influence how people explain and that the subjectivity of explaining might result in social bias. To alleviate this we call for using a large pool of annotators (implicitly increasing diversity), collecting multiple explanations, and collecting demographic attributes of annotators. In \sect{sec:collecting_highlights} and \sect{sec:related_quality} we discuss factors that influence faithfulness, i.e., how accurately explanations represent the model's decision-making process. Unfaithful explanations are at odds with the objectives of XAI outlined in \sect{sec:introduction}, one of which is quantifying bias and fairness.  
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} We include information on licenses of the datasets surveyed in \autoref{sec:appendix_license}.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We created a living version of the surveyed datasets as a website, where pull requests and issues can be opened to add and update datasets: \url{https://exnlpdatasets.github.io}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
